Adapting to Continuous Covariate Shift via Online Density Ratio Estimation

Dealing with distribution shifts is one of the central challenges for modern machine learning. One fundamental situation is the covariate shift, where the input distributions of data change from training to testing stages while the input-conditional output distribution remains unchanged. In this paper, we initiate the study of a more challenging scenario -- continuous covariate shift -- in which the test data appear sequentially, and their distributions can shift continuously. Our goal is to adaptively train the predictor such that its prediction risk accumulated over time can be minimized. Starting with the importance-weighted learning, we show the method works effectively if the time-varying density ratios of test and train inputs can be accurately estimated. However, existing density ratio estimation methods would fail due to data scarcity at each time step. To this end, we propose an online method that can appropriately reuse historical information. Our density ratio estimation method is proven to perform well by enjoying a dynamic regret bound, which finally leads to an excess risk guarantee for the predictor. Empirical results also validate the effectiveness.

==> section/related_work.tex <==
%!TEX root = ../main.tex
\section{Related Work and Discussion}
This section provides more discussions about the related work and possible directions to generalized the assumptions used in this paper.
\subsection{Related work}

\textbf{Online Distribution Shift Adaptation.} 

To the best of our knowledge, most covariate shift works focus on the one-step adaptation problem. A closely related study is~\citep{NIPS'22:Atlas}, which explores how to adapt the model to a continuous label shift. In such a situation, the label distribution $\D_t(y)$ changes over time while the label-conditional density $\D_t(\x\given y)$ remains the same. However, as discussed in Remark~\ref{remark:online-label-shift}, the previous method crucially builds on an unbiased estimator for the underlying label distribution $\D_t(y)$ to perform the importance weighted learning. However, such an unbiasedness is generally not satisfied by the density ratio estimator for covariate shift adaptation. The paper~\citep{conf/icml/JangPLB22} presented an approach for detecting covariate shift adaptation where the environments could continuously shift. The proposed method can detect the covariate shift of the streaming data with respect to the initial source data within a pre-defined sliding window. However, it is still unclear how to selectively use the historical model to update the predictor. The paper~\citep{arXiv'21:online-DRE} studied the time-varying density ratio estimation problem. Their problem setup differs from ours in that it assumes sufficient unlabeled data at each iteration $t\in[T]$. By contrast, in the online adaptation stage in our problem, the learner can only observe a limited amount of unlabeled data, which raises challenges regarding how to selectively use the historical data to train the classifier.



\textbf{Non-stationary Online Learning.}



\subsection{Discussion}

\textbf{Beyond the Linear model.}

\textbf{Beyond the Covariate Shift Assumption.}

